Theia: Distilling Diverse Vision Foundation Models for Robot Learning

Vision-based robot policy learning, which maps visual inputs to actions, necessitates a holistic understanding of diverse visual tasks beyond single-task needs like classification or segmentation. Inspired by this, we introduce Theia, a vision foundation model for robot learning that distills multiple off-the-shelf vision foundation models trained on varied vision tasks. Theia's rich visual representations encode diverse visual knowledge, enhancing downstream robot learning. Extensive experiments demonstrate that Theia outperforms its teacher models and prior robot learning models using less training data and smaller model sizes. Additionally, we quantify the quality of pre-trained visual representations and hypothesize that higher entropy in feature norm distributions leads to improved robot learning performance. Code, models, and demo are available at https://theia.theaiinstitute.com.

==> figures/feature_norm_entropy.tex <==
\begin{figure}[thbp]
    \centering
    \includegraphics[width=0.475\textwidth]{assets/norm_entropy_regular_models.png}
    \includegraphics[width=0.505\textwidth]{assets/norm_entropy_distilled_models.png}
    \caption{Feature norm entropy vs robot learning performance. We perform a linear regression analysis over each category of models and we report the Pearson correlation coefficients: R=0.954 for the regular models (left) and R=0.749 for the distilled models (right).}
    \label{fig:feature_norm_entropy}
\end{figure}

==> tables/cortexbench_all_results.tex <==
\begin{table}[htbp]
\begin{tabular}{llllll}
\toprule
Model & Head & Deterministic & Data & Note & Overall Score \\
\midrule
rvfm\_deit\_tiny\_cdsv & Conv & True & 0.1 & step00031610 & 77.27\\
rvfm\_deit\_small\_cdsv & Conv & True & 1.0 & pretrained & 76.73\\
\color{blue}{dinov2} & Conv & True & - & & 76.28\\
rvfm\_deit\_tiny\_cdsv & Conv & False & 0.1 & step00031610 & 76.08\\
\color{blue}{vith} & Conv & True & - & & 76.08\\
rvfm\_deit\_tiny\_cdsv & Conv & True & 1.0 & step00315945 & 75.70\\
rvfm\_deit\_small\_cdsv & Conv & False & 0.1 & step00031610 & 75.63\\
rvfm\_deit\_base\_cdsv & Conv & True & 0.1 & lrs\_step00031610 & 75.51\\
rvfm\_deit\_small\_cdsv & Conv & True & 0.1 & step00031610 & 75.09\\
rvfm\_deit\_base\_cdsv & Conv & True & 1.0 & lrs5\_step00063189 & 73.57\\
\color{blue}{clip} & Conv & True & - & & 73.33\\
\color{red}{vc1\_vitl\_sp} & Conv & True & vc1 & & 73.23\\
\color{red}{vc1\_vitb\_sp} & Conv & True & vc1 & & 73.00\\
rvfm\_deit\_base\_cdsv & Conv & True & 1.0  & lrs5\_step00315945 & 72.91\\
rvfm\_deit\_base\_cdsv & Conv & True & 0.1  & lrs5\_step00031610 & 72.09\\
rvfm\_deit\_small\_cdsv & Conv & True & 0.1 & lrs5\_step00031610 & 70.95\\
\color{blue}{clip+dino+vit} & Conv & True & - & - & 69.7\\
\color{red}{vc1\_vitl} & MLP & False & vc1 & & 69.39\\
\color{red}{vc1\_vitl} & MLP & True & vc1 & & 67.65\\
rvfm\_deit\_base\_cdsv & Conv & False & 0.1 & step00031610 & 67.06\\
\color{red}{vc1\_vitb} & MLP & True & vc1 & & 65.79\\
rvfm\_deit\_tiny\_cdsv & SmallConv & False & 0.1 & step00031610 & 65.65\\
\color{red}{vc1\_vitb} & MLP & False & vc1 & & 64.61\\
rvfm\_deit\_base\_cdsv & Conv & True & 0.1 & step00031610 & 60.89\\
rvfm\_deit\_tiny\_cdsv\_cls & MLP & True & 0.1 & step00031610 & 45.27\\
rvfm\_deit\_small\_cdsv\_cls & MLP & True & 0.1 & step00031610 & 38.25\\
\bottomrule
\end{tabular}
\end{table}

==> tables/target_feature_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{MuJoCo subset performance with respect of different combinations of target models. Results are all based on Theia-Tiny trained on ImageNet. C=CLIP-L, De=Depth-Anything-L, Di=DINOv2-L, S=SAM-H, V=ViT-H. All stands for the combination of all of five models, and All$-$X means taking X out of all (four models remaining).}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{c|ccccc|c|ccccc|cc}
            \toprule
            Teachers & V & C & S &Di & De & All & All$-$V & All$-$C & All$-$Di & All$-$S & All$-$De & CDiV & CDiS \\
            \midrule
            Performance & 77.37 & 76.30 & 72.36 & 72.12 & 70.40 & 76.54 & 73.96 & 74.72 & 75.45 & 76.45 & 77.89 & \textbf{78.19} & 74.12 \\
            & \multicolumn{5}{c|}{Performance ranking: V$>$C$>$S$>$Di$>$De} & ~ & \multicolumn{5}{c|}{Performance drop ranking: V$>$C$>$Di$>$0$>$S$>$De} & & \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:target_feature_ablation}
\end{table}
